A finite strain model for fiber angle plasticity of textile fabrics based on isogeometric shell finite elements

This work presents a shear elastoplasticity model for textile fabrics within the theoretical framework of anisotropic Kirchhoff-Love shells with bending of embedded fibers proposed by Duong et al. (2023). The plasticity model aims at capturing the rotational inter-ply frictional sliding between fiber families in textile composites undergoing large deformation. Such effects are usually dominant in dry textile fabrics such as woven and non-crimp fabrics. The model explicitly uses relative angles between fiber families as strain measures for the kinematics. The plasticity model is formulated directly with surface invariants without resorting to thickness integration. Motivated by experimental observations from the picture frame test, a yield function is proposed with isotropic hardening and a simple evolution equation. A classical return mapping algorithm is employed to solve the elastoplastic problem within the isogeometric finite shell element formulation of Duong et al. (2022). The verification of the implementation is facilitated by the analytical solution for the picture frame test. The proposed plasticity model is calibrated from the picture frame test and is then validated by the bias extension test, considering available experimental data for different samples from the literature. Good agreement between model prediction and experimental data is obtained. Finally, the applicability of the elastoplasticity model to 3D shell problems is demonstrated.

==> neco_updated.tex <==


\makeatletter
\DeclareRobustCommand*\ouell{\mathpalette\@ouell\relax}
\newcommand*\@ouell[2]{
  % We need to adjust the width of \uell to be the same as \ell
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.4ex \hbox{\kern \dimen0\unhbox1\kern \dimen0}}
}

\makeatletter
\DeclareRobustCommand*\houell{\mathpalette\@houell\relax}
\newcommand*\@houell[2]{
  % We need to adjust the width of \uell to be the same as \ell
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.2ex \hbox{\kern \dimen0\unhbox1\kern \dimen0}}
}

%for Gamma^\uell
%\newcommand {\uell}{\scaleto{\boldsymbol{\ouell}\mathstrut}{6.5pt}}
\newcommand {\uell}{\scaleto{{\ouell}\mathstrut}{6.5pt}}


%for L^\huell
%\newcommand {\huell}{\scaleto{\boldsymbol{\houell}\mathstrut}{6.5pt}}
\newcommand {\huell}{\scaleto{{\houell}\mathstrut}{6.5pt}}


%moving hat left
\newcommand*{\xhat}[1]{#1\kern-0.75em\hat{\phantom{#1}}}
\newcommand*{\xxhat}[1]{#1\kern0.75em\hat{\phantom{#1}}}

\newcommand {\Lhat}{\mathrm{\xhat{L}}}


\newcommand {\thetahat}{\hat{\theta}}
\newcommand {\gammahat}{\hat{\gamma}}

% Equations
\newcommand{\bitm}{\begin{itemize}}
\newcommand{\eitm}{\end{itemize}}
\newcommand{\bnumr}{\begin{enumerate}}
\newcommand{\enumr}{\end{enumerate}}
\newcommand{\bolds}[1]{\boldsymbol{#1}}
\newcommand {\nqp}{n_\mathrm{qp}}
\newcommand {\ngp}{n_\mathrm{qp}}
\newcommand {\wqp}{w_\mathrm{qp}}
\newcommand {\wgp}{w_\mathrm{qp}}

\newcommand {\sigab}{\sigma^{\alpha\beta}}
\newcommand {\ellab}{\ell^{\alpha\beta}}

\newcommand {\divv}{\mathrm{div}}
\newcommand {\smallSigma}{\scaleto{\Sigma\mathstrut}{6pt}}
\newcommand {\smallLambda}{\scaleto{\Lambda\mathstrut}{6pt}}


\newcommand {\ella}{\ell^{\alpha}}
\newcommand {\ellb}{\ell^{\beta}}

\newcommand {\nbara}{\bar{n}^{\alpha}}
\newcommand {\nbarb}{\bar{n}^{\beta}}

\newcommand {\sigbar}{\bar{\sigma}}
\newcommand {\sigmabar}{\bar{\sigma}}
\newcommand {\taubar}{\bar{\tau}}
\newcommand {\sbar}{\bar{s}}

\newcommand {\aab}{a^{\alpha\beta}}
\newcommand {\auab}{a_{\alpha\beta}}
\newcommand {\agd}{a^{\gamma\delta}}
\newcommand {\abd}{a^{\beta\delta}}
\newcommand {\abg}{a^{\beta\gamma}}
\newcommand {\aad}{a^{\alpha\delta}}
\newcommand {\aag}{a^{\alpha\gamma}}

\newcommand {\augd}{a_{\gamma\delta}}
\newcommand {\augb}{a_{\gamma\beta}}
\newcommand {\aute}{a_{\theta\epsilon}}

\newcommand {\adb}{a^{\delta\beta}}
\newcommand {\aga}{a^{\gamma\alpha}}

\newcommand {\Aab}{A^{\alpha\beta}}
\newcommand {\Auab}{A_{\alpha\beta}}
\newcommand {\Agd}{A^{\gamma\delta}}
\newcommand {\Augd}{A_{\gamma\delta}}

\newcommand {\Mab}{M^{\alpha\beta}}
\newcommand {\mab}{m^{\alpha\beta}}
\newcommand {\Mbarab}{\bar{M}^{\alpha\beta}}

\newcommand {\Mhatab}{\hat{M}^{\alpha\beta}}

\newcommand {\Mhat}{\hat{M}}

\newcommand {\mbar}{\bar{m}}
\newcommand {\mhat}{\hat{m}}


\newcommand {\Nab}{N^{\alpha\beta}}
\newcommand {\Nbarab}{\bar{N}^{\alpha\beta}}


\newcommand {\Muab}{M_{\alpha\beta}}
\newcommand {\Mgd}{M^{\gamma\delta}}
\newcommand {\Mgb}{M^{\gamma\beta}}
\newcommand {\Mugd}{M_{\gamma\delta}}

\newcommand {\bab}{b^{\alpha\beta}}

\newcommand {\buab}{b_{\alpha\beta}}
\newcommand {\baug}{b^{\alpha}_{\gamma}}
\newcommand {\bgd}{b^{\gamma\delta}}
\newcommand {\bgb}{b^{\gamma\beta}}
\newcommand {\bugd}{b_{\gamma\delta}}
\newcommand {\tbgd}{\tilde{b}^{\gamma\delta}}
\newcommand {\tauab}{\tau^{\alpha\beta}}

\newcommand{\mcalC}{\mathcal{C}}
\newcommand{\mcalS}{\mathcal{S}}

\newcommand{\mrN}{\mathrm{N}}
\newcommand{\mrD}{\mathrm{D}}
\newcommand{\mrT}{\mathrm{T}}
\newcommand{\mrL}{\mathrm{L}}
\newcommand{\bnP}{\bn_\mathrm{p}}
\newcommand{\mrin}{\mathrm{in}}



\newcommand {\eqb}[1]{\begin{equation}\begin{array}{#1}}
\newcommand {\eqe}{\end{array}\end{equation}}
\newcommand {\eqbb}[1]{\begin{equation}\boxed{\begin{array}{#1}}
\newcommand {\eqeb}{\end{array}}\end{equation}}
\newcommand {\esb}[1]{\begin{equation*}\begin{array}{#1}}
\newcommand {\ese}{\end{array}\end{equation*}}
\newcommand {\ds}{\displaystyle}
\newcommand {\ts}{\textstyle}
\newcommand {\df}[2]{\frac{\ds#1}{\ds#2}}
\newcommand {\pa}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand {\paq}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}
\newcommand {\pad}[2]{\frac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}
\newcommand {\paqq}[3]{\frac{\partial^2{#1}}{\partial{#2}\,\partial{#3}}}
\newcommand {\back}{\! \! \!}
\newcommand {\is}{\back &=& \back}
\newcommand {\dis}{\back &:=& \back}
\newcommand {\isd}{\back &=:& \back}
\newcommand {\ais}{\back &\approx& \back}
\newcommand {\isn}{\back &\neq& \back}
\newcommand {\plus}{\back &+& \back}
\newcommand {\mi}{\back &-& \back}
\newcommand {\isl}{\back &<& \back}
\newcommand {\isleq}{\back &\leq& \back}
\newcommand {\isg}{\back &>& \back}
\newcommand {\isgeq}{\back &\geq& \back}
\newcommand {\isin}{\back &\in& \back}
\newcommand {\with}{\quad,$with:$\quad}
\newcommand {\s}{~\!}

% Functions
\newcommand {\mc}[3]{\multicolumn{#1}{#2}{#3}}
\newcommand {\norm}[1]{\|#1\|}
\newcommand {\tr}{\mathrm{tr}\,}
\newcommand {\sign}{\mathrm{sign}\,}
\newcommand {\spur}{\mathrm{sp}\,}
\newcommand {\grad}{\mathrm{grad}\,}
\newcommand {\divz}{\mathrm{div}\,}
\newcommand {\rot}{\mathrm{rot}\,}
\newcommand {\Grad}{\mathrm{Grad}\,}
\newcommand {\Divz}{\mathrm{Div}\,}

% Differential
\newcommand {\dif}{\mathrm{d}}

% Average
\newcommand {\ave}[1]{\langle#1\rangle}
\newcommand {\avo}[1]{\langle #1 \rangle_{\Omega}}
\newcommand {\ava}[1]{\langle #1 \rangle_{\Omega_e}}
\newcommand {\avb}[1]{\langle #1 \rangle_{\Omega/\Omega_e}}
\newcommand {\avI}[1]{\langle #1 \rangle_{\Omega_I}}
\newcommand {\avE}[1]{\langle #1 \rangle_{\Omega_E}}
\newcommand {\iom}{\int_\Omega}
\newcommand {\pom}{\int_{\partial\Omega}}

% Invariants
\newcommand {\II}{{I\kern-.3em I}}
\newcommand {\III}{{I\kern-.3em I\kern-.3em I}}

% Integrals
\newcommand {\into}{\int_\Omega}
\newcommand {\intoo}{\int_{\Omega_0}}
\newcommand {\intI}{\int_{\Omega_I}}
\newcommand {\inta}{\int_{\Omega_1}}
\newcommand {\intb}{\int_{\Omega_2}}
\newcommand {\intc}{\int_{\Omega_3}}
\newcommand {\inti}{\int_{\Omega_i}}
\newcommand {\intj}{\int_{\Omega_j}}
\newcommand {\intk}{\int_{\Omega_k}}
\newcommand {\intl}{\int_{\Omega_\ell}}
\newcommand {\intab}{\int_{\bar{\Omega}_1}}
\newcommand {\intbb}{\int_{\bar{\Omega}_2}}
\newcommand {\intcb}{\int_{\bar{\Omega}_3}}
\newcommand {\intaob}{\int_{\bar{\Omega}_{10}}}
\newcommand {\intbob}{\int_{\bar{\Omega}_{20}}}
\newcommand {\intaobb}{\int_{\bar{\bar{\Omega}}_{10}}}
\newcommand {\intbobb}{\int_{\bar{\bar{\Omega}}_{20}}}
\newcommand {\intib}{\int_{\bar{\Omega}_i}}
\newcommand {\intjb}{\int_{\bar{\Omega}_j}}
\newcommand {\intkb}{\int_{\bar\Omega_k}}
\newcommand {\intlb}{\int_{\bar\Omega_\ell}}
\newcommand {\intie}{\int_{\Omega_i^e}}
\newcommand {\intje}{\int_{\Omega_j^e}}
\newcommand {\intpa}{\int_{\partial\bar{\Omega}_1}}
\newcommand {\intpb}{\int_{\partial\bar{\Omega}_2}}
%\newcommand {\intpi}{\int_{\partial{\Omega}_i^e}}
%\newcommand {\intpj}{\int_{\partial{\Omega}_j^e}}
%\newcommand {\intpk}{\int_{\partial{\Omega}_k^e}}
\newcommand {\intpi}{\int_{\Gamma_i^e}}
\newcommand {\intpj}{\int_{\Gamma_j^e}}
\newcommand {\intpk}{\int_{\Gamma_k^e}}
\newcommand {\intpio}{\int_{\Gamma_{i0}^{e}}}
\newcommand {\intpjo}{\int_{\Gamma_{j0}^{e}}}
\newcommand {\intpko}{\int_{\Gamma_{k0}^{e}}}

% Indices
\newcommand {\mra}{\mathrm{a}}
\newcommand {\mrb}{\mathrm{b}}
\newcommand {\mrc}{\mathrm{c}}
\newcommand {\mrd}{\mathrm{d}}
\newcommand {\mre}{\mathrm{e}}
\newcommand {\mrf}{\mathrm{f}}
\newcommand {\mrg}{\mathrm{g}}
\newcommand {\mrh}{\mathrm{h}}
\newcommand {\mri}{\mathrm{i}}
\newcommand {\mrj}{\mathrm{j}}
\newcommand {\mrk}{\mathrm{k}}
\newcommand {\mrl}{\mathrm{l}}
\newcommand {\mrm}{\mathrm{m}}
\newcommand {\mrn}{\mathrm{n}}
\newcommand {\mro}{\mathrm{o}}
\newcommand {\mrp}{\mathrm{p}}
\newcommand {\mrq}{\mathrm{q}}
\newcommand {\mrr}{\mathrm{r}}
\newcommand {\mrs}{\mathrm{s}}
\newcommand {\mrt}{\mathrm{t}}
\newcommand {\mru}{\mathrm{u}}
\newcommand {\mrv}{\mathrm{v}}
\newcommand {\mrw}{\mathrm{w}}
\newcommand {\mrx}{\mathrm{x}}
\newcommand {\mry}{\mathrm{y}}
\newcommand {\mrY}{\mathrm{Y}}

\newcommand {\mrz}{\mathrm{z}}
\newcommand {\mrP}{\mathrm{P}}
\newcommand {\mrX}{\mathrm{X}}

% Vectors (Bold lower case)
\newcommand {\ma}{\mathbf{a}}
%\newcommand {\mb}{\mathbf{b}}
\newcommand {\mcc}{\mathbf{c}}
\newcommand {\md}{\mathbf{d}}
\newcommand {\me}{\mathbf{e}}
\newcommand {\mf}{\mathbf{f}}
\newcommand {\mg}{\mathbf{g}}
\newcommand {\mh}{\mathbf{h}}
\newcommand {\mii}{\mathbf{i}}
\newcommand {\mj}{\mathbf{j}}
\newcommand {\mk}{\mathbf{k}}
\newcommand {\ml}{\mathbf{l}}
\newcommand {\mm}{\mathbf{m}}
\newcommand {\mn}{\mathbf{n}}
\newcommand {\mo}{\mathbf{o}}
\newcommand {\mpp}{\mathbf{p}}
\newcommand {\mq}{\mathbf{q}}
\newcommand {\mr}{\mathbf{r}}
%\newcommand {\ms}{\mathbf{s}}
\newcommand {\mt}{\mathbf{t}}
\newcommand {\muu}{\mathbf{u}}
\newcommand {\mv}{\mathbf{v}}
\newcommand {\mw}{\mathbf{w}}
\newcommand {\mx}{\mathbf{x}}
\newcommand {\my}{\mathbf{y}}
\newcommand {\mz}{\mathbf{z}}

\newcommand {\ba}{\boldsymbol{a}}
\newcommand {\bahat}{\boldsymbol{\hat{a}}}
\newcommand {\bghat}{\boldsymbol{\hat{g}}}

\newcommand {\bb}{\boldsymbol{b}}
\newcommand {\bbbar}{\boldsymbol{\bar{b}}}
\newcommand {\bkbar}{\boldsymbol{\bar{k}}}
\newcommand {\bbhat}{\boldsymbol{\hat{b}}}
\newcommand {\bkhat}{\boldsymbol{\hat{k}}}

\newcommand {\bKbar}{\boldsymbol{\bar{K}}}


\newcommand {\bc}{\boldsymbol{c}}
\newcommand {\bcbar}{\boldsymbol{\bar{c}}}


\newcommand {\bd}{\boldsymbol{d}}
\newcommand {\be}{\boldsymbol{e}}
\newcommand {\bff}{\boldsymbol{f}}
\newcommand {\bg}{\boldsymbol{g}}
\newcommand {\bh}{\boldsymbol{h}}
\newcommand {\bi}{\boldsymbol{i}}
\newcommand {\bj}{\boldsymbol{j}}
\newcommand {\bk}{\boldsymbol{k}}
\newcommand {\bl}{\boldsymbol{l}}
\newcommand {\blhat}{\boldsymbol{\hat{l}}}
\newcommand {\bell}{\boldsymbol{\ell}}
\newcommand {\bellhat}{{\hat{ \boldsymbol{\ell}} }}

\newcommand {\bm}{\boldsymbol{m}}
\newcommand {\bmbar}{\boldsymbol{\bar{m}}}
\newcommand {\bmhat}{\boldsymbol{\hat{m}}}
\newcommand {\bmchk}{\boldsymbol{\check{m}}}

\newcommand {\bn}{\boldsymbol{n}}
\newcommand {\bnbar}{\boldsymbol{\bar{n}}}
\newcommand {\babar}{\boldsymbol{\bar{a}}}

\newcommand {\dotbnbar}{\boldsymbol{\dot{{\bar{{n}}}}}}

\newcommand {\nbar}{\bar{n}}

\newcommand {\bo}{\boldsymbol{o}}
\newcommand {\bp}{\boldsymbol{p}}
\newcommand {\bq}{\boldsymbol{q}}
\newcommand {\br}{\boldsymbol{r}}
\newcommand {\bs}{\boldsymbol{s}}
\newcommand {\bt}{\boldsymbol{t}}
\newcommand {\bu}{\boldsymbol{u}}
\newcommand {\bv}{\boldsymbol{v}}
\newcommand {\bw}{\boldsymbol{w}}
\newcommand {\bx}{\boldsymbol{x}}
\newcommand {\bxhat}{\boldsymbol{\hat{x}}}
\newcommand {\by}{\boldsymbol{y}}
\newcommand {\bz}{\boldsymbol{z}}
%\newcommand {\bf0}{\boldsymbol{0}}
%\newcommand {\bnu}{\boldsymbol{\nu}}
\newcommand {\bmu}{\boldsymbol{\mu}}

\newcommand {\bmubar}{\boldsymbol{\bar{\mu}}}
\newcommand {\bmuhat}{\boldsymbol{\hat{\mu}}}
\newcommand {\bmuchk}{\boldsymbol{\check{\mu}}}
% Greek
\newcommand {\balp}{\mbox{\boldmath$\alpha$}}
\newcommand {\bbet}{\mbox{\boldmath$\beta$}}
\newcommand {\bdel}{\mbox{\boldmath$\delta$}}
\newcommand {\blam}{\mbox{\boldmath$\lambda$}}
\newcommand {\bnu}{\mbox{\boldmath$\nu$}}
\newcommand {\bphi}{\mbox{\boldmath$\phi$}}
\newcommand {\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand {\bvphi}{\mbox{\boldmath$\varphi$}}
\newcommand {\brho}{\mbox{\boldmath$\rho$}}
\newcommand {\bxi}{\mbox{\boldmath$\xi$}}
\newcommand {\bet}{\mbox{\boldmath$\eta$}}
\newcommand {\btheta}{\mbox{\boldmath$\theta$}}
\newcommand {\bome}{\mbox{\boldmath$\omega$}}

% 2nd Order Tensors (Bold upper case)
\newcommand {\mA}{\mathbf{A}}
\newcommand {\mB}{\mathbf{B}}
\newcommand {\mC}{\mathbf{C}}
\newcommand {\mD}{\mathbf{D}}
\newcommand {\mE}{\mathbf{E}}
\newcommand {\mF}{\mathbf{F}}
\newcommand {\mG}{\mathbf{G}}
\newcommand {\mH}{\mathbf{H}}
\newcommand {\mI}{\mathbf{I}}
\newcommand {\mJ}{\mathbf{J}}
\newcommand {\mK}{\mathbf{K}}
\newcommand {\mL}{\mathbf{L}}
\newcommand {\mM}{\mathbf{M}}
\newcommand {\mN}{\mathbf{N}}
\newcommand {\mO}{\mathbf{O}}
\newcommand {\mP}{\mathbf{P}}
\newcommand {\mQ}{\mathbf{Q}}
\newcommand {\mR}{\mathbf{R}}
\newcommand {\mS}{\mathbf{S}}
\newcommand {\mT}{\mathbf{T}}
\newcommand {\mU}{\mathbf{U}}
\newcommand {\mV}{\mathbf{V}}
\newcommand {\mW}{\mathbf{W}}
\newcommand {\mX}{\mathbf{X}}
\newcommand {\mY}{\mathbf{Y}}
\newcommand {\mZ}{\mathbf{Z}}

\newcommand {\bA}{\boldsymbol{A}}
\newcommand {\bB}{\boldsymbol{B}}
\newcommand {\bC}{\boldsymbol{C}}
\newcommand {\bD}{\boldsymbol{D}}
\newcommand {\bE}{\boldsymbol{E}}
\newcommand {\bF}{\boldsymbol{F}}
\newcommand {\bFbar}{\boldsymbol{\bar{F}}}

\newcommand {\bG}{\boldsymbol{G}}
\newcommand {\bH}{\boldsymbol{H}}
\newcommand {\bI}{\boldsymbol{I}}
\newcommand {\bJ}{\boldsymbol{J}}
\newcommand {\bK}{\boldsymbol{K}}
\newcommand {\bL}{\boldsymbol{L}}

\newcommand {\bM}{\boldsymbol{M}}

\newcommand {\bMbar}{\boldsymbol{\bar{M}}}
\newcommand {\bMhat}{\boldsymbol{\hat{M}}}
\newcommand {\bMtilde}{\boldsymbol{\tilde{M}}}
\newcommand {\bMchk}{\boldsymbol{\check{M}}}

\newcommand {\bGamma}{\boldsymbol{\Gamma}}
\newcommand {\bOmega}{\boldsymbol{\Omega}}
\newcommand {\bOmegabar}{\boldsymbol{\bar\Omega}}

\newcommand {\bGammabar}{\boldsymbol{\bar{\Gamma}}}
\newcommand {\bGammahat}{\boldsymbol{\hat{\Gamma}}}

\newcommand {\bN}{\boldsymbol{N}}
\newcommand {\bO}{\boldsymbol{O}}
\newcommand {\bP}{\boldsymbol{P}}
\newcommand {\bQ}{\boldsymbol{Q}}
\newcommand {\bR}{\boldsymbol{R}}
\newcommand {\bS}{\boldsymbol{S}}
\newcommand {\bT}{\boldsymbol{T}}
\newcommand {\bU}{\boldsymbol{U}}
\newcommand {\bV}{\boldsymbol{V}}
\newcommand {\bW}{\boldsymbol{W}}
\newcommand {\bX}{\boldsymbol{X}}
\newcommand {\bY}{\boldsymbol{Y}}
\newcommand {\bZ}{\boldsymbol{Z}}

\newcommand {\eps}{\varepsilon}
\newcommand {\sig}{\sigma}
\newcommand {\vphi}{\varphi}
\newcommand {\beps}{\mbox{\boldmath$\varepsilon$}}
\newcommand {\bLam}{\mbox{\boldmath$\Lambda$}}

\newcommand {\bsig}{\mbox{\boldmath$\sigma$}}
\newcommand {\bsigbar}{\mbox{\boldmath$\bar{\sigma}$}}


\newcommand {\bSig}{\mbox{\boldmath$\Sigma$}}
\newcommand {\btau}{\mbox{\boldmath$\tau$}}
\newcommand {\bbphi}{\mbox{\boldmath$\Phi$}}
\newcommand {\bom}{\mbox{\boldmath$\omega$}}
\newcommand {\bOme}{\mbox{\boldmath$\Omega$}}
\newcommand {\bThe}{\mbox{\boldmath$\Theta$}}
\newcommand {\bXi}{\mbox{\boldmath$\Xi$}}
\newcommand {\kd}[1]{\delta_{#1}}
\newcommand {\bone}{\mathbf{1}}
\newcommand {\bxih}{\bxi_\mathrm{h}}
\newcommand {\Boxh}{\Box_\mathrm{h}}

% 4th Order Tensors
\newcommand {\bbA}{\mathbb{A}}
\newcommand {\bbB}{\mathbb{B}}
\newcommand {\bbC}{\mathbb{C}}
\newcommand {\bbD}{\mathbb{D}}
\newcommand {\bbE}{\mathbb{E}}
\newcommand {\bbF}{\mathbb{F}}
\newcommand {\bbG}{\mathbb{G}}
\newcommand {\bbH}{\mathbb{H}}
\newcommand {\bbI}{\mathbb{I}}
\newcommand {\bbJ}{\mathbb{J}}
\newcommand {\bbK}{\mathbb{K}}
\newcommand {\bbL}{\mathbb{L}}
\newcommand {\bbM}{\mathbb{M}}
\newcommand {\bbN}{\mathbb{N}}
\newcommand {\bbO}{\mathbb{O}}
\newcommand {\bbP}{\mathbb{P}}
\newcommand {\bbQ}{\mathbb{Q}}
\newcommand {\bbR}{\mathbb{R}}
\newcommand {\bbS}{\mathbb{S}}
\newcommand {\bbT}{\mathbb{T}}
\newcommand {\bbU}{\mathbb{U}}
\newcommand {\bbV}{\mathbb{V}}
\newcommand {\bbW}{\mathbb{W}}
\newcommand {\bbX}{\mathbb{X}}
\newcommand {\bbY}{\mathbb{Y}}
\newcommand {\bbZ}{\mathbb{Z}}

\newcommand {\IR}{{\rm\kern.24em
   \vrule width.02em height1.53ex depth-.05ex
   \kern-.3em R}}
\newcommand {\ic}{{\rm\kern.20em
   \vrule width.02em height1.0ex depth-.05ex
   \kern-.22em c}}
%\newcommand {\ia}{{\rm\kern.20em
%   \vrule width.02em height1.2ex depth-.05ex
%   \kern-.32em \textit{a}}}
\newcommand {\ia}{{\rm\kern.20em
   \vrule width.02em height1.05ex depth-.0ex
   \kern-.25em a}}
\newcommand {\IC}{{\rm\kern.24em
   \vrule width.02em height1.4ex depth-.05ex
   \kern-.26em C}}
\newcommand {\ID}{{\rm\kern.34em
   \vrule width.02em height1.5ex depth-.05ex
   \kern-.36em D}}
%\newcommand {\IIo}{{\rm\kern.30em
%   \vrule width.02em height1.55ex depth-.05ex
%   \kern-.32em I}}
%\newcommand {\II}{{\rm\kern.30em
%   \vrule width.02em height1.55ex depth-.05ex
%   \kern-.32em I}_{ijkl}}
%\newcommand {\IIs}{{\rm\kern.30em
%   \vrule width.02em height1.55ex depth-.05ex
%   \kern-.32em I}^{s}_{ijkl}}
\newcommand {\IS}{{\rm\kern.24em
   \vrule width.02em height1.6ex depth.05ex
   \kern-.26em S}}
\newcommand {\IT}{{\rm\kern.50em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.52em T}}
\newcommand {\Sa}{\ds\frac{1}{2(1-\nu)}}
\newcommand {\Sb}{\ds\frac{3-4\nu}{4(1-\nu)}}
\newcommand {\Sc}{\ds\frac{1}{4(1-\nu)(3-4\nu)}}
\newcommand {\SC}{\ds\frac{1}{2(1-\nu)(3-4\nu)}}
\newcommand {\Sco}{\ds\frac{1}{4(1-\nu)(3-4\nu)R^2_0}}
\newcommand {\IE}{{\rm\kern.24em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.33em E}}
\newcommand {\IEa}{{\rm\kern.24em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.33em E}^{1}_{ijkl}}
\newcommand {\IEb}{{\rm\kern.24em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.33em E}^{2}_{ijkl}}

% Spaces
\newcommand {\sA}{\mathcal{A}}

\newcommand {\sB}{\mathcal{B}}
\newcommand {\sC}{\mathcal{C}}

\newcommand {\scrC}{\mathscr{C}}

\newcommand {\bkB}{\boldsymbol{\mathfrak{b}}}
\newcommand {\bkL}{\boldsymbol{\mathfrak{l}}}
\newcommand {\bkC}{\boldsymbol{\mathfrak{c}}}

\newcommand {\bsB}{\boldsymbol{\mathcal{B}}}
\newcommand {\bsL}{\boldsymbol{\mathcal{L}}}
\newcommand {\bsC}{\boldsymbol{\mathcal{C}}}

\newcommand {\sD}{\mathcal{D}}
\newcommand {\sE}{\mathcal{E}}
\newcommand {\sF}{\mathcal{F}}
\newcommand {\sG}{\mathcal{G}}
\newcommand {\sH}{\mathcal{H}}
\newcommand {\sI}{\mathcal{I}}
\newcommand {\sJ}{\mathcal{J}}
\newcommand {\sK}{\mathcal{K}}
\newcommand {\sL}{\mathcal{L}}
\newcommand {\sM}{\mathcal{M}}
\newcommand {\sN}{\mathcal{N}}
\newcommand {\sO}{\mathcal{O}}
\newcommand {\sP}{\mathcal{P}}
\newcommand {\sQ}{\mathcal{Q}}
\newcommand {\sR}{\mathcal{R}}
\newcommand {\sS}{\mathcal{S}}
\newcommand {\sT}{\mathcal{T}}
\newcommand {\sU}{\mathcal{U}}
\newcommand {\sV}{\mathcal{V}}
\newcommand {\sW}{\mathcal{W}}
\newcommand {\sX}{\mathcal{X}}
\newcommand {\sY}{\mathcal{Y}}
\newcommand {\sZ}{\mathcal{Z}}

\newcommand {\bsM}{\boldsymbol{\mathcal{M}}}
%vector a:
\newcommand {\vaua}{\ba_\alpha}
\newcommand {\vaa}{\ba^\alpha}

\newcommand {\vaub}{\ba_\beta}
\newcommand {\vab}{\ba^\beta}

\newcommand {\vaug}{\ba_\gamma}
\newcommand {\vag}{\ba^\gamma}

\newcommand {\vaud}{\ba_\delta}
\newcommand {\vad}{\ba^\delta}

\newcommand {\vauacb}{\ba_{\alpha,\beta}}
\newcommand {\vaugcd}{\ba_{\gamma,\delta}}

\newcommand {\vtiln}{\tilde{\bn}}
\newcommand {\vtilNcb}{\tilde{\bN}_{,\beta}}
\newcommand {\vtilNca}{\tilde{\bN}_{,\alpha}}

\newcommand {\vNcb}{\bN_{,\beta}}
\newcommand {\vNca}{\bN_{,\alpha}}
\newcommand {\vNcg}{\bN_{,\gamma}}
\newcommand {\vNcd}{\bN_{,\delta}}

\newcommand {\vNcab}{\bN_{,\alpha\beta}}
\newcommand {\vNcgd}{\bN_{,\gamma\delta}}

% Finite Elements
\newcommand{\Pint}[1]{\Pi_{\mathrm{int}#1}}
\newcommand{\Pext}[1]{\Pi_{\mathrm{ext}#1}}
\newcommand{\Pic}{\Pi_{\mathrm{c}}}
\newcommand{\fint}[1]{\mf_{\mathrm{int}#1}}
\newcommand{\fext}[1]{\mf_{\mathrm{ext}#1}}
\newcommand{\fc}[1]{\mf_{\mathrm{c}#1}}
\newcommand{\kint}[1]{\mk_{\mathrm{int}#1}}
\newcommand{\kc}[1]{\mk_{\mathrm{c}#1}}

% Coarse-Graining
%\newcommand{\mhx}{{\bf\hat\mx}}
%\newcommand{\bhx}{{\bf\hat\bx}}
%\newcommand{\mhX}{{\bf\hat\mX}}
\newcommand{\mhx}{{\mz}}
\newcommand{\mhX}{{\mZ}}

% Variations
\newcommand {\dphi}{\delta\bvphi}

% Operators
\newcommand {\Ass}[2]{\kern 0.9ex \vrule width0.45em height0.2ex depth0ex \kern -2.1ex \bigwedge_{#1}^{#2}}
\newcommand {\ASS}[2]{\kern 1.45ex \vrule width0.5em height0.2ex depth0ex \kern -2.65ex \bigwedge_{#1}^{#2}}

%tensors
\newcommand {\Cabgd}{{c}^{\alpha\beta\gamma\delta}}
\newcommand {\Dabgd}{{d}^{\alpha\beta\gamma\delta}}
\newcommand {\Eabgd}{{e}^{\alpha\beta\gamma\delta}}
\newcommand {\Fabgd}{{f}^{\alpha\beta\gamma\delta}}
\newcommand {\tCabgd}{\tilde{c}^{\alpha\beta\gamma\delta}}
\newcommand {\tDabgd}{\tilde{d}^{\alpha\beta\gamma\delta}}
\newcommand {\tEabgd}{\tilde{e}^{\alpha\beta\gamma\delta}}
\newcommand {\tFabgd}{\tilde{f}^{\alpha\beta\gamma\delta}}

\newcommand {\Babgd}{k^{\alpha\beta\gamma\delta}}
\newcommand {\babgd}{b^{\alpha\beta\gamma\delta}}

\newcommand {\cabgd}{{c}^{\alpha\beta\gamma\delta}}
\newcommand {\dabgd}{{d}^{\alpha\beta\gamma\delta}}
\newcommand {\eabgd}{{e}^{\alpha\beta\gamma\delta}}
\newcommand {\fabgd}{{f}^{\alpha\beta\gamma\delta}}


\newcommand {\mabgd}{m^{\alpha\beta\gamma\delta}}
\newcommand {\mgate}{m^{\gamma\alpha\theta\epsilon}}
\newcommand {\mdbte}{m^{\delta\beta\theta\epsilon}}
\newcommand {\mtagd}{m^{\theta\alpha\gamma\delta}}
\newcommand {\mebgd}{m^{\epsilon\beta\gamma\delta}}


% Colors
%\definecolor{col}{rgb}{0.6,0.1,0.5}

% Packed itemize
\newenvironment{packeditemize}{
\begin{itemize}
  %\setlength{\itemindent}{-10pt}
  \setlength{\listparindent}{-10pt}
  \setlength{\itemsep}{2pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}} 

